MASIM: An Efficient Multi-Array Scheduler for In-Memory SIMD Computation

Single instruction, multiple data (SIMD) is a popular design style of in-memory computing (IMC) architectures, which enables memory arrays to perform logic operations to achieve low energy consumption and high parallelism. To implement a target function on the data stored in memory, the function is first transformed into a netlist of the supported logic operations through logic synthesis. Then, the scheduler transforms the netlist into the instruction sequence given to the architecture. An instruction is either computing a logic operation in the netlist or copying the data from one array to another. Most existing schedulers focus on optimizing the execution sequence of the operations to minimize the number of memory rows needed, neglecting the energy-consuming copy instructions, which cannot be avoided when working with arrays with limited sizes. In this work, our goal is to reduce the number of copy instructions to decrease overall energy consumption. We propose MASIM, a multi-array scheduler for in-memory SIMD computation. It consists of a priority-driven scheduling algorithm and an iterative improvement process. Compared to the best state-of-the-art scheduler, MASIM reduces the number of copy instructions by 63.2% on average, which leads to a 28.0% reduction in energy.

==> 3_1_scheduler_old.tex <==
\subsection{\xadd{Random }\CombPName{}-driven \xdel{Scheduler}\xadd{Scheduling Algorithm}}\label{sec:method_sched}
The foundation of our scheduling algorithm is a priority-driven\xdel{ list} scheduler.
We say that a node is \emph{ready} if and only if all its fanins have already been computed and thus stored in the arrays.
\xadd{The overview of our scheduling algorithm is shown in left-bottom corner of Fig.~\ref{fig:overv}.}
At each time, we first evaluate the \CombPName{} priority of each ready node $n$ if it is to be scheduled in each array $A$ with a function $\textit{CalcPriority}(n,A)$ to be introduced in Section~\ref{sec:method_pri}.
\xadd{After evaluating all the $n-A$ pairs, we schedule the one that gives the highest priority by copying the missing fanins and then computing the node.}
\xdel{Then, we pick a node $n$ together with the corresponding array $A$ that gives the highest priority.
Finally, we generate the instructions to copy all fanins of $n$ that are not stored in $A$ into the rows in $A$ and then compute node $n$ in a row in $A$ according to the row picking results to be introduced in Section~\ref{sec:method_row}.}

% \begin{Example}
% We use Fig.~\ref{fig:sched} as an example to illustrate the scheduling process\xadd{, ignoring how the priority is obtained for now}.
% Initially, nodes $a$, $b$, and $c$ are stored in array $A_1$, and nodes $d$, $f$, and $h$ are stored in array $A_2$, as shown in Fig.~\ref{fig:sched}(a).
% At this moment, nodes $e$ and $g$ are ready, and we evaluate the priority of scheduling each of them in each of the two arrays\xadd{, \textit{i.e.}, $\textit{CalcPriority}(n,A)$ for $n\in\{e, g\}$ and $A\in\{A_1, A_2\}$.}
% \xadd{Suppose that }$\textit{CalcPriority}(e,A_1)$ has the highest priority\xdel{ since it does not need any copy instruction. Thus},\xadd{ so} we generate an instruction to perform the computation\xadd{, and the status of the nodes become Fig.~\ref{fig:sched}(b)}.
% Now, only node $f$ is ready, and \xadd{suppose that }$\textit{CalcPriority}(g,A_2)$ is better than $\textit{CalcPriority}(g,A_1)$\xdel{ since it has a larger \PName{} result}.
% Hence, we choose to schedule node $g$ in array $A_2$ with two instructions.
% We first copy the missing fanin $c$ into array $A_2$\xadd{, \textit{e.g.},Fig.~\ref{fig:sched}(c),} and then compute $g$ in $A_2$\xadd{, \textit{e.g.}, Fig.~\ref{fig:sched}(d)}.
% \end{Example}

\xadd{
\subsubsection{Basic Idea of \CombPName{} Priority}\label{sec:method_pridef}
In this section, we introduce the basic idea of our \CombPName{} priority.
We set minimizing the number of copy instructions that are needed to schedule the current node as our primary priority since it is the target of our scheduler.
When there is a tie in the primary priority, we turn to our secondary priority, \textit{i.e.}, maximizing the number of \PName{}s, which can give a hint on the number of copy instructions needed in the future.
As shown in Fig.~\ref{fig:mot}(b), we say that node $n$ and node $i$ are \emph{partners} of each other if they share a fanout $x$ that has not been computed yet.
If the two nodes are stored in the same array $A_1$, we say that they form a \emph{close partner pair} (\PName{}) in array $A_1$.
We favor memory status with a large number \PName{}s since it indicates that the scheduled nodes which will be used to perform a computation are more likely to be stored in the same array, thus requiring less copy instructions in the future.
To maximize the number of \PName{}s, we maximize the change of the number when making the decisions.
We use $\textit{NPA}(n,A)$ to denote the number of partners of node $n$ stored in array $A$.
When node $n$ emerges in array $A$ by copying or computing, the number of \PName{}s increase $\textit{NPA}(n,A)$.
When node $n$ is overwritten in array $A$, the number of \PName{}s decreases $\textit{NPA}(n,A)$.

\begin{figure}[!htbp]
    \centering
    \includegraphics[scale=0.32]{sched_ex.png}
    \caption{Scheduling example: (a) initial state; (b) compute $e$ in $A_1$; (c) copy $c$ to $A_2$; (d) compute $g$ in $A_2$.}
    \label{fig:sched}
\end{figure}

\begin{Example}
We use Fig.~\ref{fig:sched} as an example to illustrate the \CombPName{} priority, supposing that both arrays, \textit{i.e.}, $A_1$ and $A_2$, have enough empty rows.
In the initial status in Fig.~\ref{fig:sched}(a), nodes $e$ and $g$ are ready and can be scheduled in array $A_1$ or array $A_2$.
Among the four node-array pairs, scheduling node $e$ in array $A_1$ does not need any copy instruction, while the other choices need 1 or 2 copy instructions.
Thus, we decide to schedule $e$ in array $A_1$ by generating a computation instruction, and the status of the nodes becomes Fig.~\ref{fig:sched}(b).
Now, only node $f$ is ready, and scheduling it in array $A_1$ and array $A_2$ both need one copy instruction, so we need to use the secondary priority.
$\textit{NPA}(g,A_2)=2$ since two partners of node $g$, \textit{i.e.}, nodes $f$ and $h$, are stored in $A_2$.
Similarly, we can obtain $\textit{NPA}(g,A_1)=1$.
Therefore, we choose to schedule $f$ in $A_2$ since it has larger change in the number of \PName{}s and potentially needs less copy instructions in the future.
We first copy the missing fanin $c$ into array $A_2$, \textit{e.g.},Fig.~\ref{fig:sched}(c), and then compute $g$ in $A_2$, \textit{e.g.}, Fig.~\ref{fig:sched}(d).
Starting from the memory status in Fig.~\ref{fig:sched}(d), we require one copy instruction to compute node $i$ and node $j$, \textit{i.e.}, copying node $e$ to array $A_2$.
However, if we schedule $f$ in $A_1$, we will require two copy instructions.
This observation confirms the strength of our secondary priority.
\end{Example}

In this example, the two priorities seem to be easy to obtain.
However, this is only because we assume that the arrays have enough empty rows so we can use arbitrary rows to store the copied fanins and the computation results of the nodes.
In the real case, the arrays are filled with results of the computed nodes so we must carefully pick the rows according to the \CombPName{} priority.}

\subsubsection{Node Priority Calculation}\label{sec:method_pri}

\begin{algorithm}[!htbp]
\caption{Node priority calculation.}
\label{algo:pri}
\begin{small}
\KwData{$(\#\textit{copy}, \Delta\textit{TLOC}\xadd{, S})\leftarrow\textit{CalcPriority}(n, A)$}
\KwIn{$n$: a node in netlist.
$A$: an array.}
\KwOut{$\#\textit{copy}$: number of copy instructions and $\Delta\textit{TLOC}$: the change in total \PName{} required to schedule $n$ in $A$.
\xadd{$S$: scheduling result.}
}
$\#\textit{copy}\leftarrow0; \Delta\textit{TLOC}\leftarrow0\xadd{; S\leftarrow \emptyset}$\;\label{A1:init}
\ForEach{fanin $i$ of $n$}
{\label{A1:fanin}
    \If{$i$ is not in $A$}
    {\label{A1:fanin_if}
        $(R, C, L)\leftarrow\textit{PickRow}(A, \textit{True})$\;\label{A1:fanin_row}
        \lIf{$R=\emptyset$}{\Return{$(-1,0, \emptyset)$}}\label{A1:fanin_fail}
        $\#\textit{copy}\leftarrow\#\textit{copy}+C+1$\;\label{A1:fanin_copy}
        $\Delta\textit{TLOC}\leftarrow\Delta\textit{TLOC}+L+\textit{Loc}(i,A)$\;\label{A1:fanin_loc}
        \xadd{$S\leftarrow \{i: R\}\bigcup S$\;}\label{A1:sched_copy}
    }
}
$(R, C, L)\leftarrow\textit{PickRow}(A, \textit{True})$\;\label{A1:res_row}
\lIf{$R = \emptyset$}{\Return{$(-1,0, \emptyset)$}}\label{A1:res_fail}
$\#\textit{copy}\leftarrow\#\textit{copy}+C$\;\label{A1:res_copy}
$\Delta\textit{TLOC}\leftarrow\Delta\textit{TLOC}+L+\textit{Loc}(n,A)$\;\label{A1:res_loc}
\xadd{$S\leftarrow \{n: R\}\bigcup S$\;}\label{A1:sched_compute}
\Return{$(\#\textit{copy}, \Delta\textit{TLOC}\xadd{, S})$}\;\label{A1:ret}
\end{small}
\end{algorithm}

Now, we illustrate how to obtain the priority of scheduling node $n$ in array $A$ with the function $\textit{CalcPriority}(n, A)$, whose pseudo code is shown in Algorithm~\ref{algo:pri}.
As mentioned above, our primary priority is minimizing the number of copy instructions ($\#\textit{copy}$) needed to compute node $n$ in array $A$, and our secondary priority is maximizing the change in total \PName{} ($\Delta\textit{TLOC}$).
Hence, these two metrics are returned as the output of the function, and they are initialized to 0 in Line~\ref{A1:init}.

Since we can only compute an operation on the rows within the same array, we must copy all fanins of the operation that are not in array $A$ to array $A$ before passing the computation instruction.
The algorithm traverses all fanins of node $n$ (Line~\ref{A1:fanin}).
If a fanin $i$ is not in array $A$ (Line~\ref{A1:fanin_if}), Line~\ref{A1:fanin_row} calls a function $\textit{PickRow}$ to pick a row in array $A$ to store the copied $i$.
The function $\textit{PickRow}$ will be introduced in Section~\ref{sec:method_row}.
Its outputs are row picking result $R$, the number of copy instructions $C$, and the change in total \PName{} $L$ needed when emptying the picked row.
Note that here we say that we \emph{empty} the picked row does not mean that we actually need to delete the stored data in the row.
Instead, we make the data redundant and can be overwritten so that we can use the row to hold other data.
Then, Line~\ref{A1:fanin_copy} increases $\#\textit{copy}$ by $(C+1)$ since it needs $C$ copy instructions to empty the picked row and one copy instruction to copy $i$ to the picked row.
Moreover, Line~\ref{A1:fanin_loc} increases $\Delta\textit{TLOC}$ by $(L+\textit{Loc}(i,A))$ since the change in total \PName{} is $L$ when emptying the picked row and $\textit{Loc}(i,A)$ when copying $i$ to $A$.
\xadd{Line~\ref{A1:sched_copy} adds the row picking result $R$ for fanin $i$ to the scheduling result.}
After copying all missing fanins to $A$, Line~\ref{A1:res_row} picks a row to hold the result of the node $n$.
$\#\textit{copy}$ and $\Delta\textit{TLOC}$ are increased by $C$ and $(L+\textit{Loc}(n,A))$, respectively, in Lines~\ref{A1:res_copy}--\ref{A1:res_loc}\xadd{, and the row picking result for node $n$ is also put into the scheduling result in Line~\ref{A1:sched_compute}}.
During the process, when $\textit{PickRow}$ fails to pick a row in array $A$, \textit{i.e.}, $R=\emptyset$, the algorithm returns $\#\textit{copy}=-1$ (see Lines~\ref{A1:fanin_fail} and~\ref{A1:res_fail}). 

\subsubsection{Row Picking Strategy}\label{sec:method_row}
\begin{algorithm}[!htbp]
\caption{Row picking strategy.}
\label{algo:row}
\begin{small}
\KwData{$(R, \#\textit{copy}, \Delta\textit{TLOC})\leftarrow\textit{PickRow}(A, \textit{canCopy})$}
\KwIn{$A$: the array to pick row from.
$\textit{canCopy}$: whether allowing copying when picking the row.}
\KwOut{$R$: row picking result.
$\#\textit{copy}$: the number of copy instructions.
$\Delta\textit{TLOC}$: the change in total \PName{}.}
\If{there exists free row $r$ in array $a$}
{\label{A2:free1}
\Return{$(\{A: r\}, 0, 0)$}\;\label{A2:free2}
}
$\textit{maxTLOC} \leftarrow -\infty; R\gets\emptyset$\;\label{A2:init}
\ForEach{duplicated node $d$ stored in row $r$ of array $A$}
{\label{A2:dup}
$\textit{L}\leftarrow -\textit{Loc}(d,A)$\;\label{A2:dup_loc}
\lIf{$L>\textit{maxTLOC}$}{$\textit{maxTLOC}\leftarrow L; R\gets\{A: r\}$}\label{A2:dup_choose}
}
\lIf{$\textit{maxTLOC}\neq -\infty$}
{\Return{$(R, 0, \textit{maxTLOC})$}}\label{A2:dup_ret}
\lIf{$\textit{canCopy}$ is $\textit{False}$}
{\Return{$(\emptyset, 0, 0)$}}\label{A2:canCopy_ret}
\ForEach{array $A'\neq A$}
{\label{A2:undup}
    $(R', \#\textit{copy}', \Delta\textit{LOC}')\leftarrow\textit{PickRow}(A', \textit{False})$\;\label{A2:undup_pickpick}
    \If{$R'\neq\emptyset$}
    {\label{A2:undup_pickcheck}
        \ForEach{node $n$ stored in row $r$ of array $A$}
        {\label{A2:undup_node}
            $\textit{TotL}\leftarrow Loc(n,A')+\Delta\textit{LOC}'-\textit{Loc}(n,A)$\;\label{A2:undup_loc}
            \If{$\textit{TotL}>maxLOC$}
            {\label{A2:undup_choose1}
            $\textit{maxTLOC}\leftarrow \textit{TotL}; R\gets\{A: r\}\bigcup R'$\;\label{A2:undup_choose2}
            }
        }
    }
}
\lIf{$\textit{maxTLOC}\neq -\infty$}
{\Return{$(R, 1, \textit{maxTLOC})$}}\label{A2:undup_ret}
\Return{$(\emptyset, 0, 0)$}\;\label{A2:ret}
\end{small}
\end{algorithm}

Now, we illustrate how to pick a row in array $A$ that will be emptied to store the copied fanin or the computed node result.
The row picking strategy is implemented with a function $\textit{PickRow}$, whose pseudo code is shown in Algorithm~\ref{algo:row}.
We introduce a flag $\textit{canCopy}$ as an input of the function $\textit{PickRow}$ to denote whether we allow for the inserting of copy instructions when emptying the picked row.
The flag $\textit{canCopy}$ is set to true when calling the function in Algorithm~\ref{algo:pri} and set to false when recursively calling the function to avoid infinite loops.
The meaning of the outputs is explained in Section~\ref{sec:method_pri}, and we will illustrate the row picking strategy using the example in Fig.~\ref{fig:row_ex}.

\begin{figure}[!htbp]
    \centering
    \includegraphics[scale=0.3]{row_ex.png}
    \caption{Row picking strategy example: (a) case 1; (b) case 2; (c) case 3.}
    \label{fig:row_ex}
\end{figure}

Since the copy instruction and \PName{} change when picking the row will be accumulated in the priority function as illustrated in Section~\ref{sec:method_pri}, we also aim to minimize $\#\textit{copy}$ and then maximize $\Delta\textit{TLOC}$ for $\textit{PickRow}$.
Under this target, there are three cases with decreasing priority:

Case 1 (Lines~\ref{A2:free1}--\ref{A2:free2}): This is the ideal case where there are free rows in the array as shown in Fig.~\ref{fig:row_ex}(a).
A row is said to be \emph{free} if there is no node stored in that row or the stored node is no longer needed.
For example, in Fig.~\ref{fig:sched}(b), after computing node $e$ in array $A_1$, the results of node $a$ and node $b$ are no longer needed and can be overwritten without any cost, \textit{i.e.}, \PName{} reduction, so the rows storing their results are regarded as free rows.
In this case, Line~\ref{A2:free2} returns $\#\textit{copy}=0$ and $\Delta\textit{TLOC}=0$.

Case 2 (Lines~\ref{A2:init}--\ref{A2:dup_ret}): This is the case where there is no free row in the array, but there are duplicated nodes stored in the array as shown in Fig.~\ref{fig:row_ex}(b).
A node is said to be \emph{duplicated} if 1) it is needed for the future computation, \textit{i.e.}, it is a PO or has fanouts that have not been computed yet, and 2) it is stored in more than one array.
For example, in Fig.~\ref{fig:sched}(c), node $c$ is duplicated since it has a fanout $g$ that has not been computed yet, and it is stored in both arrays $A_1$ and $A_2$.
Ideally, we avoid overwriting a duplicated node in an array, since we may need to compute its fanouts in that array.
However, when there is no free row in an array, we have to pick a row that stores a duplicated node and overwrite the row.
\xadd{We pick the row so that the change in \PName{} is maximized.
The maximum value is denoted as $\textit{maxTLOC}$, which is initialized in Line~\ref{A2:init}.}
When overwriting a duplicated node $d$ in array $A$, the change in the total \PName{} is $L = -\textit{Loc}(d,A)$ as evaluated in Line~\ref{A2:dup_loc}.
Line~\ref{A2:dup_choose} uses $L$ to update $\textit{maxTLOC}$\xdel{ as the maximum $L$}, and Line~\ref{A2:dup_ret} returns $\#\textit{copy}=0$ and $\Delta\textit{TLOC}=\textit{maxTLOC}$.

Cases 3 (Lines~\ref{A2:undup}--\ref{A2:undup_ret}): This is the worst case where there is no free row and all nodes stored in the array are not duplicated, as shown in Fig.~\ref{fig:row_ex}(c).
In this case, if we want to pick a row $r$, we need to first insert a copy instruction to copy the stored node $n$ to another array $A'$.
Hence, if we do not allow copying in $\textit{PickRow}$, \textit{i.e.}, $\textit{canCopy}$ is false,
Line~\ref{A2:canCopy_ret} returns the row picking result as empty before checking for case 3.
Line~\ref{A2:undup} traverses each array $A'$ ($A' \neq A$), and Line~\ref{A2:undup_pickpick} picks a row in $A'$ to store the node to be copied from array $A$ with a recursive call of function $\textit{PickRow}$ with the flag $\textit{canCopy}$ set to false.
When a row can be picked from $A'$ (Line~\ref{A2:undup_pickcheck}), Line~\ref{A2:undup_node} further traverses each node $n$ stored in row $r$ of array $A$.
The change in total \PName{} when copying node $n$ to array $A'$ and emptying row $r$ is $Loc(n,A')+\Delta\textit{LOC}'-\textit{Loc}(n,A)$, where $\Delta\textit{LOC}'$ is the change in \PName{} when picking the row in $A'$.
Lines~\ref{A2:undup_choose1}--\ref{A2:undup_choose2} keep the result with the maximum change in \PName{}, which is returned together with $\#\textit{copy}=1$ in Line~\ref{A2:undup_ret}.
